A Method to Translate Order-Sorted Algebras to Many-Sorted Algebras

Order-sorted algebras and many sorted algebras exist in a long history with many different implementations and applications. A lot of language specifications have been defined in order-sorted algebra frameworks such as the language specifications in K (an order-sorted algebra framework). The biggest problem in a lot of the order-sorted algebra frameworks is that even if they might allow developers to write programs and language specifications easily, but they do not have a large set of tools to provide reasoning infrastructures to reason about the specifications built on the frameworks, which are very common in some many-sorted algebra framework such as Isabelle/HOL, Coq and FDR. This fact brings us the necessity to marry the worlds of order-sorted algebras and many sorted algebras. In this paper, we propose an algorithm to translate a strictly sensible order-sorted algebra to a many-sorted one in a restricted domain by requiring the order-sorted algebra to be strictly sensible. The key idea of the translation is to add an equivalence relation called core equality to the translated many-sorted algebras. By defining this relation, we reduce the complexity of translating a strictly sensible order-sorted algebra to a many-sorted one, make the translated many-sorted algebra equations only increasing by a very small amount of new equations, and keep the number of rewrite rules in the algebra in the same amount. We then prove the order-sorted algebra and its translated many-sorted algebra are bisimilar. To the best of our knowledge, our translation and bisimilar proof is the first attempt in translating and relating an order-sorted algebra with a many-sorted one in a way that keeps the size of the translated many-sorted algebra relatively small.

==> eptcsdata.tex <==
\providecommand{\firstpage}{20}
\providecommand{\publicationstatus}{H. Cirstea, D. Sabel (Eds.): Fourth International Workshop on Rewriting\\
Techniques for Program Transformations and Evaluation (WPTE 2017)\\
EPTCS 265, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.265.3}{10.4204/EPTCS.265.3}}

